Vector boson pair production at one loop: analytic results for the process $q \bar{q} \ell \bar\ell \ell^\prime \bar{\ell}^\prime g$

We present compact analytic results for the one-loop amplitude for the process $0 \rightarrow q \bar{q} \ell \bar\ell \ell^\prime \bar{\ell}^\prime g$, relevant for both the production of a pair of $Z$ and $W$-bosons in association with a jet. We focus on the gauge-invariant contribution mediated by a loop of quarks. We explicitly include all effects of the loop-quark mass $m$, appropriate for the production of a pair of $Z$-bosons. In the limit $m \to 0$, our results are also applicable to the production of $W$-boson pairs, mediated by a loop of massless quarks. Implemented in a numerical code, the results are fast. The calculation uses novel advancements in spinor-helicity simplification techniques, for the first time applied beyond five-point massless kinematics. We make use of primary decompositions from algebraic-geometry, which now involve non-radical ideals, and $p$-adic numbers from number theory. We show how to infer whether numerator polynomials belong to symbolic powers of non-radical ideals through numerical evaluations.

==> qloop_b127_asy.tex <==
\begin{eqnarray}
&&b^{(0,A)}_{\{127\}}=\Bigg\{
\frac{\spa1.5\*\spa1.7\*\spa5.7\*s_{127}\*\tspbaba4.12.34.56.3}
{2\*\spa1.2\*s_{34}\*\spa5.6
\*\spaba7.12.56.7^2\*\spab7.12.7}
\nonumber\\&&
+\frac{\spb2.7\*\spa5.7\*s_{127}\*(\spa1.3\*\spb4.6\*s_{56}
-2\*\spa1.5\*\spa3.7\*\spb4.7\*\spb5.6
-\spa1.3\*\spb4.6\*s_{567})}
{4\*s_{34}\*s_{56}\*\spab7.12.7^2\*\spaba7.12.56.7}
\nonumber\\&&
+\spb2.7
\*\frac{(\spa1.7\*\spa3.5\*\spb4.6\*s_{56}
+\spa1.3\*\spb4.6\*\spaba5.34.12.7
-2\*\spa1.5\*\spa3.5\*\spa3.7\*\spb3.4\*\spb5.6)}
{4\*s_{34}\*s_{56}\*\spab7.12.7\*\spaba7.12.56.7}
\nonumber\\&&
-\spa1.3
\*\frac{(\spa1.3\*\spab5.34.6-\spa1.5\*\spa3.5\*\spb5.6)\*(s_{127}-s_{56})}
{2\*\spa1.2\*\spa3.4\*\spaba7.12.56.7\*\Delta_3(3,4,5,6)}
\nonumber\\&&
-\frac{\spa1.3\*(3\*\spa1.3\*\spb3.4\*\spab5.34.6
+\spab1.56.4\*\spab5.34.6
+4\*\spb3.4\*\spa3.5\*\spab1.34.6)}
{2\*\spa1.2\*\spaba7.12.56.7\*\Delta_3(3,4,5,6)}
\nonumber\\&&
+\frac{\spa1.5\*\spb4.6\*\spab1.56.4\*(s_{127}-s_{56})}
{2\*\spa1.2\*\spb3.4\*\spaba7.12.56.7\*\Delta_3(3,4,5,6)}\Bigg\}
-\Bigg\{\;\Bigg\}_{3 \leftrightarrow 5,4 \leftrightarrow 6}
\end{eqnarray}


==> qloop_b12_asy.tex <==
\begin{eqnarray}
&&b^{(0,A)}_{\{12\}}=\Bigg\{
\frac{\spb1.2\*\spa1.5\*\spa1.7\*\spa5.7\*\tspbaba4.12.34.56.3}
{2\*s_{34}\*\spa5.6\*\spab7.12.7\*\spaba7.12.56.7^2}
\nonumber\\&&
+\spa5.7\*\spb2.7\*s_{12}
\*\frac{(\spa1.3\*\spb4.6\*s_{567}
-\spa1.3\*\spb4.6\*s_{56}
+2\*\spa1.5\*\spa3.7\*\spb4.7\*\spb5.6)}
{4\*s_{34}\*s_{56}\*\spab7.12.7^2\*\spaba7.12.56.7}
\nonumber\\&&
+\spa1.3\*\spb2.7\*\frac{(
-\spb4.6\*\spaba5.34.12.7
-2\*\spa5.7\*\spbab4.34.12.6
+\spb4.6\*\spa5.7\*(s_{567}-s_{34}))}
{4\*s_{34}\*s_{56}\*\spab7.12.7\*\spaba7.12.56.7}
\nonumber\\&&
+\frac{(-2\*\spa1.3\*\spb2.4\*\spaba5.12.34.5
-\spa3.5\*\spab1.34.2\*\spab5.12.4
-2\*\spa1.5\*\spab3.12.4\*\spab5.67.2)}
{2\*\spa5.6\*\spaba7.12.56.7\*\Delta_3(1,2,3,4)}
\nonumber\\&&
+\spa3.5
\*\frac{(4\*\spa1.2\*\spb1.2\*\spa1.5\*\spb2.4
-3\*\spa1.2\*\spb2.4\*\spab5.34.2
-\spb1.2\*\spa1.3\*\spa1.5\*\spb3.4)}
{2\*\spa5.6\*\spaba7.12.56.7\*\Delta_3(1,2,3,4)}
\\&&
-\frac{\spa1.3\*\spa3.5\*\spab5.67.2\*(s_{12}-s_{567}+s_{34})}
{2\*\spa3.4\*\spa5.6\*\spaba7.12.56.7\*\Delta_3(1,2,3,4)}
+\frac{\spa1.5\*\spb2.4\*\spab5.12.4\*(s_{12}-s_{567}+s_{34})}
{2\*\spb3.4\*\spa5.6\*\spaba7.12.56.7\*\Delta_3(1,2,3,4)}
\Bigg\}
-\Bigg\{\;\Bigg\}_{3\leftrightarrow5,4\leftrightarrow6}\nonumber
\end{eqnarray}


==> qloop_bub127_old.tex <==
\begin{eqnarray}
b^{(0)}_{\{127\}}&=&\Big[\Big\{\frac{-\spa1.7^2\*\spa5.7^2\*s_{127}
\*\spab7.12.4^2\*\spbab7.12.56.7}
{\spa1.2\*\spb3.4\*\spa5.6\*\spab7.12.7^2
\*\spaba7.12.56.7^3}
\nonumber\\
&+&\frac{3\*\spa1.7\*\spb2.7\*\spb4.7\*\spa5.7^2
\*s_{127}\*\spab7.12.4}
{2\*\spb3.4\*\spa5.6\*\spab7.12.7^2
\*\spaba7.12.56.7^2}
\nonumber\\
&+&\frac{\spa1.5\*\spa1.7\*\spb4.7\*\spa5.7\*\spab7.12.4}
{2\*\spa1.2\*\spb3.4\*\spa5.6
\*\spaba7.12.56.7^2}
\nonumber\\
&-&\frac{\spa1.7\*\spa5.7\*\spab7.12.4
\*(\spb2.7\*\spab5.36.4+\spb1.2\*\spa1.5\*\spb4.7)}
{\spb3.4\*\spa5.6\*\spab7.12.4
\*\spaba7.12.56.7^2}
\nonumber\\
&-&\frac{\spa1.7}
{\spa1.2\*\spaba7.12.56.7^2\*\Delta_3(3,4,5,6)}
\*\left(\frac{\spab1.27.4\*\spab5.34.4
\*\spab7.12.4\*(s_{56}-s_{127})}
{\spb3.4}\right)
\nonumber\\
&+&\frac{\spa1.7}
{\spa1.2\*\spaba7.12.56.7^2\*\Delta_3(3,4,5,6)}
\*\left(\frac{\spa1.5\*\spa5.7\*\spab3.56.4\*s_{127}
\*(s_{34}-s_{127})}
{\spa5.6}\right)
\nonumber\\
&-&\frac{\spbab1.56.27.1}
{\spa1.2\*\spaba7.12.56.7\*\Delta_3(3,4,5,6)}
\*\left(\frac{\spb4.6^2\*\spa5.6}
{\spb3.4}
+\frac{\spb3.4\*\spa3.5^2}
{\spa5.6}\right)
\nonumber\\
&-&\frac{\spa1.3\*\spa1.7\*\spab7.12.4
\*\spab5.34.4\*(s_{456}-s_{356})}
{\spa1.2\*\spaba7.12.56.7^2\*\Delta_3(3,4,5,6)}\Big\}
+\Big\{\;\Big\}_{3 \leftrightarrow 5,4 \leftrightarrow 6}
\nonumber\\
&-&\frac{\spa1.7\*\spab3.56.4\*\spab5.34.4
\*(3\*\spa1.7\*s_{127}+2\*\spaba1.35.12.7)}
{\spa1.2\*\spaba7.12.56.7^2\*\Delta_3(3,4,5,6)}
\nonumber\\
&-&\frac{4\*\spbab1.56.27.1
\*(3\*\spab3.56.4\*\spab5.34.4\*s_{127}
+\spa3.5\*\spb4.6\*\Delta_3(3,4,5,6))}
{\spa1.2\*\spaba7.12.56.7\*\Delta_3(3,4,5,6)}\Big]
\end{eqnarray}


==> qloop_d12x34x56m0_old.tex <==
\begin{eqnarray}
\label{d12x34x560}
d_{\{12\sep34\sep56\}}^{(0)}=&&-\frac{1}{4}
\*\Bigg[\bigg\{\big(\spa5.7\*\spab7.12.4\*\spaba7.56.34.1\big)^2\bigg\}
+\bigg\{\;\bigg\}_{1 \leftrightarrow 5,2 \leftrightarrow 6}\Bigg]\nonumber\\
&\times&\frac{(s_{127}\*s_{567}-s_{12}\*s_{56})}
{\spa5.6\*\spa1.2\*\spb3.4\*\spaba7.56.12.7^4}
\end{eqnarray}


==> qloop_d56x12x34m0.tex <==
\begin{eqnarray}
d_{\{56\sep12\sep34\}}^{(0)}=&&-\frac{1}{4}
\*\Bigg[\bigg\{\big(\spa3.7\*\spab7.56.2\*\spaba7.34.12.5\big)^2\bigg\}
+\bigg\{\;\bigg\}_{3 \leftrightarrow 5,4 \leftrightarrow 6}\Bigg]\nonumber\\
&\times&\frac{(s_{347}\*s_{567}-s_{34}\*s_{56})}
{\spb1.2\*\spa3.4\*\spa5.6\*\spaba7.34.56.7^4}
\end{eqnarray}


==> qloop_dt12x56x34m2_old.tex <==
\begin{eqnarray}
&&\tilde{d}_{\{12\sep56\sep34\}}^{(2)}=\frac{1}
{2\*s_{12}\*s_{34}\*s_{56}}\*\Bigg[
\frac{\Big(2\*\spa1.7\*\spa5.3\*\spb2.7\*\spb6.7\*\spb4.7\*s_{12}\Big)}
{\spab7.12.7}
\nonumber\\&&
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)}
{\spab7.12.7^2\*\spaba7.34.12.7}\*\Big(
\spa1.2\*\spa5.7\*\spa3.7\*\spb2.7^2\*\spb6.4\*s_{12}
-\spa1.7\*\spa5.7\*\spb2.7\*\spb6.4
\*\spab3.12.7\*s_{12}\Big)
\nonumber\\&&
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)}
{\spab7.12.7^2\*\spaba7.34.12.7}\*\Big(
-\spa1.2\*\spa1.5\*\spa3.7\*\spb1.2
\*\spb2.7\*\spb6.4\*\spab7.12.7
+\spa1.5\*\spa1.7\*\spb1.2\*\spb6.4
\*\spab3.12.7\*\spab7.12.7
\nonumber\\&&\qquad
-\spa1.7^2\*\spa5.3\*\spb1.2\*\spb6.7\*\spb4.7\*s_{12}
-\spa1.7\*\spa5.3\*\spb2.7\*\spb6.7
\*\spab7.12.4\*s_{12}\Big)
\nonumber\\&&
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)}
{\spab7.12.7\*\spaba7.34.12.7}\*\Big(
-\spa1.2\*\spa1.7\*\spa5.3\*\spb1.2\*\spb2.6\*\spb4.7
-\spa1.2\*\spa5.3\*\spb2.6\*\spb2.7\*\spab7.12.4
+\spa1.5\*\spa3.7\*\spb2.7\*\spb6.4\*s_{12}
\nonumber\\&&\qquad
+\spa1.7\*\spa5.3\*\spb2.6\*\spb4.7\*s_{12}
-\spa1.7\*\spa5.3\*\spb2.7\*\spb4.7\*\spab7.12.6\Big)
\nonumber\\&&
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)}
{\spab7.12.7\*\spbab7.12.34.7}
\*\spa1.2\*\spa5.3\*\spb2.7^2\*\spb6.7\*\spb4.7
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)}
{\spaba7.34.12.7}
\*\spa1.7\*\spa5.3\*\spb2.6\*\spb4.7
\nonumber\\&&
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)^2\*\spa1.7}
{\spab7.12.7^2\*\spaba7.34.12.7^2}\*\Big(
\spa1.2\*\spa5.7\*\spa3.7\*\spb1.2\*\spb2.7\*\spb6.4
+\spa1.7\*\spa5.3\*\spb1.2\*\spb4.7\*\spab7.12.6
\nonumber\\&&
-\spa1.7\*\spa5.7\*\spb1.2\*\spb6.4\*\spab3.12.7
+\spa5.3\*\spb2.7\*\spab7.12.6\*\spab7.12.4\Big)
\nonumber\\&&
+\frac{\left(s_{127}\*s_{347}-s_{12}\*s_{34}\right)^2\*\spa1.7}
{\spab7.12.7\*\spaba7.34.12.7^2}
\*\Big(\spa1.5\*\spa3.7\*\spb1.2\*\spb6.4
-\spa5.3\*\spb2.6\*\spab7.12.4\Big)
+2\*\spa1.2\*\spa5.3\*\spb2.6\*\spb2.7\*\spb4.7\Bigg]
\end{eqnarray}

